symQV: Automated Symbolic Verification of Quantum Programs

We present symQV, a symbolic execution framework for writing and verifying quantum computations in the quantum circuit model. symQV can automatically verify that a quantum program complies with a first-order specification. We formally introduce a symbolic quantum program model. This allows to encode the verification problem in an SMT formula, which can then be checked with a delta-complete decision procedure. We also propose an abstraction technique to speed up the verification process. Experimental results show that the abstraction improves symQV's scalability by an order of magnitude to quantum programs with 24 qubits (a 2^24-dimensional state space).

==> reviews/fmcad.tex <==
SUBMISSION: 13
TITLE: symQV: Automated Symbolic Verification of Quantum Programs


----------------------- REVIEW 1 ---------------------
SUBMISSION: 13
TITLE: symQV: Automated Symbolic Verification of Quantum Programs
AUTHORS: Fabian Bauer-Marquart, Stefan Leue and Christian Schilling

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
Summary:
The paper presents a modeling approach of quantum programs and their properties as an SMT formula, and then a solver determines whether a given property holds. The technique first models a cubit with as tuple of four symbolic variables over real numbers with an initial set of constraints over their input domains. Next, each quantum gate is modeled as operation on those symbolic qubits. Since the resulting formulas contain non-linear operations, besides exact solution the technique is also extended to compute approximate formulas. Both versions of the technique are evaluated on several quantum programs with different number of qubits and type of input state space.

Pros:
+ Novel modeling of quantum programs over symbolic qubit
+ Nice evaluations
Cons:
- Many concepts are not well explained, formal definitions and examples are inconsistent
- The paper is difficult to follow, and some concepts are not well explained
- No examples on how such model looks as an SMT formula

Evaluation:
The paper proposes a novel idea on how to symbolically model qubits, i.e., inputs/outputs of quantum programs, as well as quantum gates over those symbolic qubits. I really liked the evaluation that show interesting results, like depending on the type of the program simulators might be a preferred choice. Evaluations also provide nice insights into the scalability of the exact and approximated symQV.

However, I find the paper is quite difficult to follow, and I don’t feel that there are enough details or justification provided for a particular modeling approach. For example, why a qubit model needs 4 tuples? Since there is a relation between the amplitude variables \alpha and \beta, and the phase angle variable \theta, \phi, then why not represent qubit just with one or another pair? If \alpha_I does not have imaginary part, then why we cannot model \alpha as a real?

While having two running concrete examples is wonderful, I would rather prefer the paper to focus on just Teleportation, but explain the modeling in details, e.g., show concretely how its states are represented in S. Otherwise, I find some inconsistencies between Definition 1 and the instance description of Teleportation example. The definition states that a sequence operation is a pair of a matrix/map and a sequence of input qubits, and in the example, there are just sequences of matrices. Are those parameters to matrices are the input qubits?  Also, in the model in ->, should be a parenthesis before Ucx on b0 and b1? In addition, here both b0 and b1 have concrete valuations in V0, then why are they in the symbolic qubit set of Q? Adding those explanations would greatly improve the understanding on the framework. I still have difficult time understand how measurement matrices fit in the sequence – are those connect s3 and sF states?

The paper states that those models are translated into an SMT formula. However, it does not describe how those formulas are being created, or giving an actual SMT formulas (even for a simplest cubit/gate program). Listings of high-level codes are not sufficient; they just re-iterate the high-level modeling. 

The paper needs to discuss whether such modeling is automated, and if not, then could it be done. The paper also needs to add discussion on what type of properties could it verify and whether there are restrictions?

In summary, I like the paper’s novelty and evaluations, but the current presentation hinders understanding and reproducing the presented technique.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 13
TITLE: symQV: Automated Symbolic Verification of Quantum Programs
AUTHORS: Fabian Bauer-Marquart, Stefan Leue and Christian Schilling

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
The paper presents a framework (called symQV) for formally verifying properties of quantum circuits. In this framework, the verification problem is encoded as an SMT problem (that is solved with the SMT-solver dReal). More precisely, each gate is modeled either via matrix multiplication or via a mapping between qubits; for example, applying a SWAP gate on a pair of qubits q_i and q_j can be encoded either via matrix multiplication with the state-vector, or via a mapping (|q_i>, |q_j>) -> (|q_j>, |q_i>) that swaps the state of the two qubits. In general, mappings lead to more concise SMT encodings but can only be applied under restricted conditions. The property is written in first-order logic. The paper uses two over-approximation techniques to make verification more scalable: the so-called "delta-relaxation" and approximating the Bloch sphere by a cube. The techniques are illustrated on two examples (quantum teleportation and Grover's diffusion operator), and two more exampl
es are described in the appendix. Last but not least, the symQV tool has an easy-to-use Python API for specifying quantum circuits and properties.

As quantum computers are now becoming a reality, formal verification of quantum programs is becoming an important problem that needs better algorithms and tools. I feel that the paper makes a solid contribution here, and would like to see it accepted. The paper is generally well-written.


Detailed Comments / Questions:

- [Specifying properties]. I would like to see a more detailed discussion on how to come up with the right specifications of a quantum program. For instance, for the quantum teleportation example, the considered specification is that the initial state of qubit |psi> is equal to the final state of qubit |b1>. This is certainly a necessary property of quantum teleportation, but it does not seem to be sufficient. A circuit that just applies a SWAP gate between |psi> and |b1> would also satisfy the given specification, but can hardly be considered as implementing teleportation. Additionally, I intuitively expect a specification stating that at the end the qubit |b1> is not entangled with other qubits. I also suggest to explicitly include specifications in the description of the running examples (on page 3).    

- [Mapping vs. matrix]. How much representing gates as mappings and not by matrices (whenever possible) contributes in terms of runtime? Quoting the paper: "Only when necessary, for example when qubits become entangled, do we construct the state vector for this specific subset of qubits". Intuitively, I expect most of the qubits to be entangled throughout an algorithm. Do you have any data for the number of gates that are represented using mappings vs. matrices? How would the runtimes change if only matrix multiplication was used? I would have also liked to see the teleportation example worked out in more detail, describing the actual created SMT formula (in particular, illustrating what gets implemented as a matrix and what as a mapping) in addition to / instead of Listing 1. 

- Please provide a few more details about delta-relaxation. 

- Do I understand correctly that for all of the experiments (listed in Tables II and III), the verification results are UNSAT, despite delta-relaxation and over-approximation?

- In Running Example II, you say: "For the remainder of this paper, we use Grover’s diffusion operator (GDO) as a running example". This sentence is a bit strange, as you use two running examples throughout the paper.


***UPDATE AFTER REBUTTAL***

I have not changed my opinion that the work is interesting and worth publishing, however after reading the rebuttal I am now even more convinced that the problem of coming up with the right specifications of quantum programs is far from being trivial, possibly explaining why other works focus on a clearer task of verifying compiler optimizations. I agree that this is an "art, just as for common programs", yet I have significantly more intuition what the correct properties are for the "common programs", and almost no intuition for the "quantum programs", in particular what the "other specifications" might be for the teleportation example and whether the presented approach would be able to verify these.

By lowering the score, I only mean that the paper is not quite ready in the current form, but I would love to see all these details worked out and the paper eventually published.



----------------------- REVIEW 3 ---------------------
SUBMISSION: 13
TITLE: symQV: Automated Symbolic Verification of Quantum Programs
AUTHORS: Fabian Bauer-Marquart, Stefan Leue and Christian Schilling

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
This paper introduces a new tool called symQV, which is a symbolic execution engine capable of analyzing quantum programs that aims to deliver similar results to equivalent tools for traditional software. This new tool can analyze up to 24 qubits. The paper uses overapproximation techniques in analyzing the matrices required to simulate quantum programs to increase tractability and enable analysis of quantum programs via symbolic execution. The presented algorithm is SMT-based, which is a feature. 

I did not see whether the tool symQV is available anywhere. For reproducibility and future-use purposes, it is essential to include information as to where to find the tool prominently; I suggest a \thanks{} at the end of the paper title with the URL for symQV.

The topic of quantum computing is far outside my area of expertise; I know much more about symbolic execution. It is not clear to me whether 24 qubits is a good size or not. The paper compares to a tool that can analyze 300 qubits with restrictions on the inputs so it seems that unrestricted inputs significantly impacts the number of qubits? I find it hard to judge the contributions with respect to quantum computing. 

The abstract mentions “delta-complete” and “delta-relaxation” as major details of the paper’s contributions but neither of these two terms appear anywhere in the introduction. If they are important to the paper, they need to be mentioned (with intuitive definitions and citations) in the introduction. Otherwise, the abstract needs to be revised to match the contributions in the introduction. Similarly, the abstract mentions that this paper pertains to the context of the “quantum gate model” but the introduction does not define that either, or frame the contributions in that context. 

The abstract, or introduction, or both, need to expand the acronym in the tool name symQV.

The paper is generally well-organized. The summary of shortcomings of related work in the introduction does a nice job of framing the gap in the current state of the art that this paper aims to address. 

As someone who is not an expert in quantum computing, I appreciated the clear Background section, but still had to look up some terms, like I presume the set \mathcal{C} is the set of complex numbers?

Importantly, the abstract and Section 5 talk about delta values (and varying these frames the experiments in Section 5) yet Section 2 does not clearly explain what these are or what their impact is on the eventual results. In section 5, what does it mean to “use the delta value of 10^{-4}” and what is the significance of varying the precision levels of delta?

The results in Section 5 appear in two large tables. Even with the accompanying text, it is not at all clear how significant they are or what, exactly, they mean. I have trouble judging the quality or coverage of the benchmarks used in the experiments (perhaps due to lack of familiarity with quantum computing), but the paper also needs to do a better job of putting this in context. The results need to be in graphs, not tables, which show the relationships between the different experiments clearly. Why do we have a whole column labeled “simulation” that is filled in with “n/a” on every row?

All figures need more descriptive captions that tell the reader what we are looking at and what the take-away messages are. For example Figure 2’s and 5’s captions need to tell us what the colors mean (I presume they do more than just highlight the three axes?). Also, given the prevalence of red-green colorblindness, I recommend changing one of those two colors. In Figure 3, what is the symbol in the boxes labeled M1 and M2? (For example, the caption for Table 1 is nice; my only comment on that is that the “which” needs to be a “that” to correct the grammar.)

Where do the 12 labeled Encodings come from? Is this a comprehensive list from a previous work on quantum computing or a set of representative examples?

It would be clearer and more consistent if the paper labeled “Running Example 1” the same way throughout; like make pages 3 and 5 match. (Same comment for Running Example 2.)

Why was dReal chosen as the SMT solver? There are many options for SMT solvers; it would be very helpful to know how interchangeable this choice is. What parameters constrain which SMT solvers would work here? Also, this information would best appear early in the paper, such as in the introduction, so that we know the options before Section 4. 

I appreciate that the proof of Theorem 1 appears in the appendix. I strongly request that the proofs for Theorems 2 and 3 be expanded similarly. The proof of Theorem 3 is simply “This follows from Theorem 2 and [35].” Yet, Theorem 3 is quite important, central to the paper’s results, and relates the output of the SMT solver to the given algorithm in a way that is not obvious just given Theorem 2 and a citation. 


Typos and other small errors:
throughout: “i.e.” and “e.g.” always need to be followed by commas as in “i.e.,” and “e.g.,”
throughout: “which” is descriptive (and often preceded by a comma) whereas “that” is restrictive — many instances of “which” should be “that” like:
— pg 1: paradigm which -> paradigm that
throughout: I’ve been told that “counter-example” is an example of a counter but “counterexample” is what a model checker returns
throughout: in English, do not capitalize the word after a colon; errors include:
— abstract: contributions: First
— pg 1: symbolically: The
throughout: commas go inside closing quotation marks; errors include:
— pg 1: “search space*,*” (comma needs to be inside as shown)
throughout: please do not start a sentence with a citation but start with a word instead
pg 1: “automated quantum program verification:” needs to end in a period instead of a colon (it’s the end of a sentence!)
pg 1: “Existing tools either*:*” (needs a :)
pg 2: “can be summarized as follows:” needs a period instead of a colon
pg 3: “allows to reason about” (e.g., replace with “allows reasoning about”)



----------------------- REVIEW 4 ---------------------
SUBMISSION: 13
TITLE: symQV: Automated Symbolic Verification of Quantum Programs
AUTHORS: Fabian Bauer-Marquart, Stefan Leue and Christian Schilling

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
This paper presents SymQV, a symbolic execution framework for writing and verifying quantum programs. Using SymQV, programmers can verify quantum programs by writing first order logic specifications over the program input and output.  The main contributions of the paper are the symbolic quantum programming model and their over-approximation technique to speed up the verification of quantum programs.

This is interesting work.  As far as I know, it is novel as claimed by the authors.  And there are some promising initial results.

However, the presentation is unclear and not self-contained in many places. Also, the over-approximation technique seems fairly course.  It relaxes qubits' degrees of freedom from the unit sphere to the unit cube.  Additionally, they drop the matrix representation in the encoding for some computations, which only works when there is no entanglement.

What are the limitations on the types of programs that can be verified?

“The first technique is an over-approximation ... The second technique can, in fact, do without
the matrix ...”
It was a little unclear where these techniques were defined. The over-approximation was obvious, but the other technique is not explicitly pointed out later, although I believe it’s encoding 2.

Nit: “[21–25] propose using interactive proof assistants to verify quantum programs.” - I find this format is less readable than naming the authors or the work and citing at the end.

Figure 3 could use a little more explanation; the bending lines are a little confusing. They should go into a little more detail about what a controlled gate is. They do not mention that it means the state of the control influences whether the operation is performed on the target.

Encoding 2 for gate mapping needs more explanation - why exactly is this okay?

In section 4, they show soundness and completeness, and they give examples of the verification code. There is a brief description of the over-approximation, which relaxes the qubits' degrees of freedom. This section feels rushed and could benefit from elaboration.

Why are there no counter-examples in the evaluation section? / Why were no incorrect programs used for the benchmarks?

In the evaluation, I’d like to see the range of the 10 runs in order to understand if there’s much variability in runtime.

Table 2 - The authors could do a better job explaining why the exact SMT solving does better on some problems and why the simulation is so much faster for most of the problems where they can compare their work to Qiskit simulation.

Table 3 - why so stable after a certain level of precision?

Section 6 has a typo: “because the state space grows *which* (with) every input variable added to the program.”

==> reviews/tacas.tex <==
# Review 1

problem focus and motivation	Quantum computing has recently gained momentum in various application
domains, including safety-critical ones. Therefore, it is important to
meet the safety specifications. To this end, this paper proposes
QuAVL, an automated verification and repair approach based on logic
encoding for quantum programs.
technical contribution	The proposed technique represents safety specifications by first-order
logic formulae. Then, it leverages a delta-complete decision procedure
over the reals to verify and repair the quantum programs under
analysis.
literature	Although I am not an expert, it seems that the paper does discuss
necessary literature on the subject.
presentation	The current presentation shall be further improved to make the paper
easier to follow:

- The current version does not introduce the basics about quantum
programs, and directly starts with quantum program modeling.

- The current version does not have concrete examples to illustrate
the proposed technique, making it very hard to follow.

- The writing shall also be further improved. For example, for
"Compared to existing fully automated verification methods such as
Amy, 2019 [20]...", unfortunately, there is only some Amy 2018 work
cited, and [20] is another different work.
Overall evaluation	
-1: (weak reject)
On the positive side, this paper works on a very important problem,
quantum program verification and repair, and can potentially inspire
more work in the same direction. The current evaluation results also
demonstrate the effectiveness of the proposed technique.

In the meantime, besides the above mentioned presentation issues, I
also have the following suggestions for further improving this work:

The program repair portion is one key contribution of this
work. However, the description is minimal and unclear. Also, the paper
directly targets two types of errors without further discussion and
justification. It would be better if the paper can further 1) what are
the other types of common errors for quantum programs, and 2) why
these 2 types have been selected as the targets.

The experiments section is also not well organized or justified. For
example, some of the example case studies have repair results while
some don't. Also, it is not clear how the benchmark programs are
selected from [27] since the [27] website has included more programs.

In the literature, researchers have proposed various other techniques
for verifying quantum programs. However, the paper only compares the
proposed technique against [28] (published 8 years ago). It is not
quite clear why more recent techniques (such as [3]) were not
considered in the experimental study.
comments to authors	I liked the vision of the work. In the meantime, it would be great if
the paper presentation and experimental evaluation can be further
improved to make this work stronger.

---

# Review 2

problem focus and motivation	This paper aims to develop an automated technique for proving correctness properties of quantum programs, as well as repairing those programs when the specification does not hold.
technical contribution	The paper makes the following contributions:

- A model of the semantics of quantum programs, including those that use (some) entanglement, suitable for encoding as an SMT problem. The model mostly attempts to leverage a non-entangled qubit representation, to keep the state space small.

- An approach to program repair using the above encoding. The approach introduces one or more *ansatz* circuits whose gates have unspecified parameters; the verification procedure will fill these in during solving, with non-identity solutions constituting a repair.

- An implementation leveraging a d-satisfiability solver over the Reals (dReal).

- Experimental results on a handful of programs illustrating capability and performance. These include proper quantum programs (teleportation and QFT) but also many that are just (classical) reversible circuits (Sec 5.4).

The program repair technique is most interesting/novel, but I question its utility. The model and verification are not improving on the state of the art, in terms of capability.
literature	Some key comments are left out of the discussion of related work:

- One important prior paper is not discussed: Nengkun Yu and Jens Palsberg, Quantum Abstract Interpretation, PLDI'21. https://dl.acm.org/doi/10.1145/3453483.3454061. This paper also describes a fully automatic software analysis technique, but to my mind takes a more principled and general approach to the question of abstraction, and it works on programs that exhibit more significant entanglement, e.g., GHZ state preparation and Grover's algorithm.

- Amy's path-sums technique "Towards Large-scale Functional Verification of Universal Quantum Circuits" is mentioned, but not entirely fairly. Amy was able to verify the same programs as those listed in the paper, and more, for equally large sizes. Path sums directly represent arbitrary quantum states, contrasting the submitted paper's collection of representations and abstractions (which are hard to follow, precisely). It is fair that Amy cannot do program repair, but nevertheless I feel that while bullet 4 of the introduction is technically true, it is misleading.

- The submitted paper is not able to abstract the number of qubits, e.g., to verify QFT for an arbitrary number of qubits; the "forall" is only with regard to initial qubit values. QBRicks and SQIR (both cited), though only partially automated, support (and have done) such proofs. The submitted paper's technique scales exponentially in the number of qubits, so such abstraction capabilities seem critical to its future success, even if they may warrant human intervention. This point should be conceded to give the reader the full picture.
presentation	The presentation could be improved.

Sometimes symbols are used without definition. More importantly, the choice of presenting a "model" first, and then a "SAT encoding" second is confusing, because some important connections that would be useful for understanding the first are not mentioned until presenting the second. The representation of entangled states, and the methods used for abstraction, I found in particular to be short on detail.

I don't think this work could be reproduced from the description. More specifics on the comments below.
Overall evaluation	
-2: (reject)
I do not believe this paper, in its current form, makes a significant enough contribution to warrant publication at a strong conference. I just didn't learn much from reading this paper, and I think the long-term future of the ideas is questionable.

- It is not clear how/whether the SAT encoding will scale. There is not enough detail about abstraction and entanglement for others to build on. For that matter, the uncited Yu and Palsberg paper arguably has developed a better, more principled technique.

- The program repair technique is a nice idea, but is inadequately motivated and evaluated. The evaluated QFT algorithm is simple and well understood; I would like to see more novel/interesting algorithms with bugs, or ones previously identified as buggy. What happens as the circuit sizes scale up and algorithms diversify?
comments to authors	General suggestion: Present this model more top-down, and integrate it with your SAT encoding. Indicate the model components first. The explain those components, referring back to the overall model to say how the pieces fit together. Better yet: Prove your encoded model is sound and complete with respect to a standard semantics of quantum programs.

Detailed comments:

Encoding 1: $|\alpha|^2 + |\beta|^2 = 1$. Instead of using $z$ as the metavariable to introduce the encoding for complex numbers, and then $\alpha$ and $\beta$ for qubits, why not use greek variables form the start?

Encoding 3: What is $k$? Defining the mapping as $\mathcal{H}^k_2 \mapsto \mathcal{H}^k_2, Q \mapsto Q'$ is confusing; perhaps this means that you represent them with matrices, when entanglement is possible, and as qubit mappings otherwise? Encodings 7-8 talk about matrix representations, but do not connect back to this earlier definition.

Encoding 9: I did not understand what's going on in this encoding. What is the $\circ$ operator? What does the $Q_f \in \{ ... \}$ signify? I'm not sure why constant vs. balanced qualifiers are indicated here---an oracle could be *any* classical function, right?

Encoding 10: Symbols $M...$ are not explained, so I'm not sure how they are used. The multiple subscripts are not explained. The use of states $s$ and probabilities $p$ is not foreshadowed---we don't know what they are for, or how they are to be used.

Definition 1: The sequence of states $S$ is confusing to me. Are you saying that the "model" needs to enumerate all intermediate states in executing the quantum program? Is this synthesized during verification (I hope so!)? How? I find the latter part of the definition, starting at the bullet list, to be confusing.

Verification section: This seems like it's making connections that the reader would have already figured out by reading section 2. The soundness/completeness result seems obvious. A more interesting result would be to prove that your initial model is indeed equivalent to the more traditional presentation of quantum computing, e.g., using density matrices.

The representation of entanglement also belongs in section 2. Indeed, it's not clear how one moves from the non-entangled to entangled representations (and back). The paper does not discuss it carefully, but this is a very important part of any automated approach.

Evaluation:

For 5.2, the suggestion seems to be that you have to run this algorithm with two particular oracles, rather than a symbolic representation of the two classes; if I'm wrong, please clarify how you specify $U_f$.

For 5.3, in the specification: What does subscript $(i,F)$ refer to? What is the notation $[0.x_i...x_n]$ mean in the exponent of the $e$ term? You are missing the $|1>$ basis state on this term.

For 5.4: Why only a subset of these benchmarks? Since they involve classical functions, why do we care?

---

# Review 3

problem focus and motivation	This paper presents QuVAL, an SMT-based verification and repair approach for quantum programs.
technical contribution	The main contributions of this paper are as follows:
1. A way of encoding a quantum program as an SMT query.
2. Repairing quantum program against two types of error.
3. Experiments comparing QuAVL with other algorithms.
literature	yes
presentation	The paper was easy to follow and nice to read.
Overall evaluation	
-2: (reject)
Unfortunately, there are several points that require significantly more work from the authors:


1. No explanation of why it is enough to consider encoding of only these
gates.

2. Even for programs with just 12 qubits, it can take a very long time
as shown in the example
of the Deutsch-Jozsa algorithm. Also, adding a lot of X gates can
increase the number of gates
but it doesn't increase the complexity of the problem very much.

3. It encodes full matrices and state vectors when qubits are entangled,
which is a huge
and common problem in simulating quantum computers on classical
computers. Could there be better
encoding for entangled qubits, e.g construct matrix, and the state
vector only for the entangled
qubits and represent other qubits same as before.

4. Why is precision error important? I think the main motive is to
verify quantum programs which
would run on an actual quantum computer.

5. The most promising part of the paper was repairing but its
explanation requires more attention.
Also, can you look at errors like "wrong gate" in which a correct gate
is replaced by a wrong gate?

6. In [28], the benchmark 'add64-ncv-h' takes time 16.23 seconds,
whereas in this paper it is
reported as 301.97 seconds. Why is there such a huge difference?
comments to authors	I appreciate the effort of the authors to convey the ideas in an understandable manner and encourage them to resubmit after they address the points above.

==> trash.tex <==
Next, we prove that the verifier's soundness is preserved when using the over-approximation.

\begin{theorem}[Over-approximation soundness]
    \Cref{enc:qubit-over-approx} preserves soundness with respect to specification verification.
\end{theorem}

\begin{proof}
    Suppose we apply \Cref{enc:qubit-over-approx} to the qubits which form the program's quantum state. 
    Next, we conduct specification verification, i.e. the encoding of the quantum program model $\qmodel$ and the specification's negation $\neg \varphi$ are combined to obtain $\qmodel \land \neg \varphi$.
    For verification, we have to distinguish two cases:
    \begin{enumerate}
        \item The verifier returns \unsat, meaning for all reachable states, including the states newly included by the over-approximation, the quantum program model $\qmodel$ satisfies the specification $\varphi$. 
        Therefore, this is also true for the concrete case and soundness is preserved.
        \item The verifier returns $\delta$-\sat{} and a counter-example.
        If the counter-example is outside Hilbert space, we have encountered a spurious counter-example not present in the concrete quantum program. Repeating the verification without the over-approximation is necessary.
        If the counter-example is in Hilbert space, the counter-example is also present in (a $\delta$-relaxation of) the concrete quantum program and we can terminate.
        \hfill \qedhere
    \end{enumerate}
\end{proof}
